Parametric estimation for convolutionally observed diffusion processes

We propose a new statistical observation scheme of diffusion processes named convolutional observation, where it is possible to deal with smoother observation than ordinary diffusion processes by considering convolution of diffusion processes and some kernel functions with respect to time parameter. We discuss the estimation and test theories for the parameter determining the smoothness of the observation, as well as the least-square-type estimation for the parameters in the diffusion coefficient and the drift one of the latent diffusion process. In addition to the theoretical discussion, we also examine the performance of the estimation and the test with computational simulation, and show an example of real data analysis for one EEG data whose observation can be regarded as smoother one than ordinary diffusion processes with statistical significance.

==> preamble.tex <==
\usepackage[a4paper,top=3cm,bottom=3cm,left=2.5cm,right=2.5cm,marginparwidth=1.75cm]{geometry}

% order of citations
% https://tex.stackexchange.com/questions/190842/same-author-same-year-bibliography-order
\newcommand{\GG}[1]{}


% maketitle
\usepackage[UKenglish]{babel}

% math fonts and symbols
\usepackage{amsfonts,amsmath,amsthm,amssymb} % \text and \mathbb command
\usepackage[foot]{amsaddr}
\usepackage{mathrsfs} % script type font
\usepackage{stmaryrd} % new bracket
\usepackage{mathtools}

% Bernoulli Journal
\RequirePackage[OT1]{fontenc}
\usepackage{natbib}

\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% others
\usepackage{comment} % commenting out multiple lines
\usepackage{graphicx} % graphics
\usepackage{setspace}
\usepackage{color}

\usepackage{multirow}

\allowdisplaybreaks[1]
%\setlength\parindent{15pt}

\newtheorem{theorem}{Theorem}%[subsection]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{remark}
\newtheorem{remark}{Remark}

